Observability of Sensorless Electric Drives

Electric drives control without shaft sensors has been an active research topic for almost three decades. It consists of estimating the rotor speed and/or position from the currents and voltages measurement. This paper deals with the observability conditions of electric drives in view of sensorless control. The models of such systems are strongly nonlinear. For this reason, a local observability approach is applied to analyze the deteriorated performance of sensorless drives in some operating conditions. The validity of the observability conditions is confirmed by numerical simulations and experimental data, using an extended Kalman filter as observer.

==> IJC_2016_GS.tex <==
-        Affiliation : je crois qu’il faut rajouter Université Parsi saclay à la fin pour le L2S.

-        Page 3 : the real problem lies in the observability conditions of the drive [Holtz, 2002]. à the real problem relies on the observability conditions of the drive [Holtz, 2002].

-        Ne manqué-t-il pas l’echelle sur les courbes d’erreur de position (fig. 27 et 30), où on voit des erreurs de position de 20 rad ? C’était pareil dans la thèse, mais ca ne m’avait pas frappé ?
